High Altitude Platform Stations: the New Network Energy Efficiency Enabler in the 6G Era

The rapidly evolving communication landscape, with the advent of 6G technology, brings new challenges to the design and operation of wireless networks. One of the key concerns is the energy efficiency of the Radio Access Network (RAN), as the exponential growth in wireless traffic demands increasingly higher energy consumption. In this paper, we assess the potential of integrating a High Altitude Platform Station (HAPS) to improve the energy efficiency of a RAN, and quantify the potential energy conservation through meticulously designed simulations. We propose a quantitative framework based on real traffic patterns to estimate the energy consumption of the HAPS integrated RAN and compare it with the conventional terrestrial RAN. Our simulation results elucidate that HAPS can significantly reduce energy consumption by up to almost 30\% by exploiting the unique advantages of HAPS, such as its self-sustainability, high altitude, and wide coverage. We further analyze the impact of different system parameters on performance, and provide insights for the design and optimization of future 6G networks. Our work sheds light on the potential of HAPS integrated RAN to mitigate the energy challenges in the 6G era, and contributes to the sustainable development of wireless communications.

==> 2_related.tex <==
\section{Related Work}
% delete and move in introduction
...

==> rtc.tex <==
@ARTICLE{lopezperez2022survey,
  author={L\'opez–P\'erez, David and De Domenico, Antonio and Piovesan, Nicola and Xinli, Geng and Bao, Harvey and Qitao, Song and Debbah, Merouane},
  journal={IEEE Communications Surveys and Tutorials}, 
  title={{A Survey on 5G Radio Access Network Energy Efficiency: Massive MIMO, Lean Carrier Design, Sleep Modes, and Machine Learning}}, 
  year={2022},
  volume={24},
  number={1},
  pages={653-697}}
  
  @article{shehab20215g,
  title={{5G networks towards smart and sustainable cities: A review of recent developments, applications and future perspectives},
  author={Shehab, Muhamma}d J and Kassem, Ihab and Kutty, Adeeb A and Kucukvar, Murat and Onat, Nuri and Khattab, Tamer},
  journal={IEEE Access},
  volume={10},
  pages={2987--3006},
  year={2021},
  publisher={IEEE}
}

@article{pouttu20206g,
  title={{6G white paper on validation and trials for verticals towards 2030’s}},
  author={Pouttu, Ari and Burkhardt, Frank and Patachia, Christian and Mendes, Luciano and Brazil, Germany Romania and Pirttikangas, Susanna and Jou, Emery and Kuvaja, Pasi and Finland, Finland Taiwan and Heikkil{\"a}, Marjo and others},
  journal={6G Research Visions},
  volume={4},
  year={2020}
}

@article{yang20196g,
  title={{6G wireless communications: Vision and potential techniques}},
  author={Yang, Ping and Xiao, Yue and Xiao, Ming and Li, Shaoqian},
  journal={IEEE network},
  volume={33},
  number={4},
  pages={70--75},
  year={2019},
  publisher={IEEE}
}

@article{mahdi20215g,
  title={{From 5G to 6G technology: meets energy, internet-of-things and machine learning: a survey}},
  author={Mahdi, Mohammed Najah and Ahmad, Abdul Rahim and Qassim, Qais Saif and Natiq, Hayder and Subhi, Mohammed Ahmed and Mahmoud, Moamin},
  journal={Applied Sciences},
  volume={11},
  number={17},
  pages={8117},
  year={2021},
  publisher={MDPI}
}

@article{kurt2021vision,
  title={{A vision and framework for the high altitude platform station (HAPS) networks of the future}},
  author={Kurt, Gunes Karabulut and Khoshkholgh, Mohammad G and Alfattani, Safwan and Ibrahim, Ahmed and Darwish, Tasneem SJ and Alam, Md Sahabul and Yanikomeroglu, Halim and Yongacoglu, Abbas},
  journal={IEEE Communications Surveys \& Tutorials},
  volume={23},
  number={2},
  pages={729--779},
  year={2021},
  publisher={IEEE}
}

@article{alam2021high,
  title={{High altitude platform station based super macro base station constellations}},
  author={Alam, Md Sahabul and Kurt, Gunes Karabulut and Yanikomeroglu, Halim and Zhu, Peiying and D{\`a}o, Ngoc D{\~u}ng},
  journal={IEEE Communications Magazine},
  volume={59},
  number={1},
  pages={103--109},
  year={2021},
  publisher={IEEE}
}

@techreport{3gpp.38.811,
  author = "{3rd Generation Partnership Project; Technical Specification Group Radio Access Network}",
  title = "{{Study on New Radio (NR) to support non-terrestrial networks (Release 15)}}",
  institution = "{3rd Generation Partnership Project (3GPP)}",
  type = "{Technical Report}",
  number = "{38.811}",
  version = "{15.4.0}",
  year = "{2020}",
  month = "{September}",
  url = "{https://portal.3gpp.org/desktopmodules/Specifications/SpecificationDetails.aspx?specificationId=3234}"
}

@article{piovesan2022machine,
  title={{Machine Learning and Analytical Power Consumption Models for 5G Base Stations}},
  author={Piovesan, Nicola and L{\'o}pez-P{\'e}rez, David and De Domenico, Antonio and Geng, Xinli and Bao, Harvey and Debbah, M{\'e}rouane},
  journal={IEEE Communications Magazine},
  volume={60},
  number={10},
  pages={56--62},
  year={2022},
  publisher={IEEE}
}

@misc{5gamericas,
  author = {5G Americas},
  title = {{Understanding mmWave Spectrum for 5G Networks}},
  howpublished = {White Paper},
  year = {2017},
  note = {Available at \url{https://www.5gamericas.org/wp-content/uploads/2020/12/InDesign-Understanding-mmWave-for-5G-Networks.pdf}}
}

@inproceedings{shibata2019study,
  title={{A study on cell configuration for HAPS mobile communications}},
  author={Shibata, Yohei and Kanazawa, Noboru and Hoshino, Kenji and Ohta, Yoshichika and Nagate, Atsushi},
  booktitle={2019 IEEE 89th Vehicular Technology Conference (VTC2019-Spring)},
  pages={1--6},
  year={2019},
  organization={IEEE}
}

@article{jia2022hierarchical,
  title={{Hierarchical aerial computing for internet of things via cooperation of HAPs and UAVs}},
  author={Jia, Ziye and Wu, Qihui and Dong, Chao and Yuen, Chau and Han, Zhu},
  journal={IEEE Internet of Things Journal},
  year={2022},
  publisher={IEEE}
}

@article{shah2021adaptive,
  title={{Adaptive-combining-based hybrid FSO/RF satellite communication with and without HAPS}},
  author={Shah, Suyash and Siddharth, Mokkapati and Vishwakarma, Narendra and Swaminathan, R and Madhukumar, AS},
  journal={IEEE Access},
  volume={9},
  pages={81492--81511},
  year={2021},
  publisher={IEEE}
}

@article{jia2021toward,
  title={{Toward Data Collection and Transmission in 6G Space--Air--Ground Integrated Networks: Cooperative HAP and LEO Satellite Schemes}},
  author={Jia, Ziye and Sheng, Min and Li, Jiandong and Han, Zhu},
  journal={IEEE Internet of Things Journal},
  volume={9},
  number={13},
  pages={10516--10528},
  year={2021},
  publisher={IEEE}
}

@misc{3gppSimulation,
  author = "3GPP TSG-RAN WG4",
  title = "Simulation assumptions for HAPS co-existence, 3GPP TSG-RAN WG4 Meeting \#100-e, Electronic Meeting",
  month = aug,
  year = "2021",
  url = "https://www.3gpp.org/ftp/tsg_ran/WG4_Radio/TSGR4_100-e/Inbox/Chairman_Notes/RAN4_100-e_Main_session_report_11_Fri_Sep_03_EOM_after_post-meeting.docx"
}

@misc{earth_d,
  author = {Gunther Auer and Oliver Blume and Vito Giannini and Istvan Godor and Muhammad Ali Imran and Ylva Jading and Efstathios Katranaras and Magnus Olsson and Dario Sabella and Per Skillermark and Wieslawa Wajda},
  title = {{Energy efficiency analysis of the reference systems, areas of improvements and target breakdown, INFSO-ICT-247733 EARTH Deliverable D2.3}},
  year = {2010},
  url = {https://cordis.europa.eu/docs/projects/cnect/3/247733/080/deliverables/001-EARTHWP2D23v2.pdf}
}
